Worst-case Delay Bounds in Time-Sensitive Networks with Packet Replication and Elimination

Packet replication and elimination functions are used by time-sensitive networks (as in the context of IEEE TSN and IETF DetNet) to increase the reliability of the network. Packets are replicated onto redundant paths by a replication function. Later the paths merge again and an elimination function removes the duplicates. This redundancy scheme has an effect on the timing behavior of time-sensitive networks and many challenges arise from conducting timing analyses. The replication can induce a burstiness increase along the paths of replicates, as well as packet mis-ordering that could increase the delays in the crossed bridges or routers. The induced packet mis-ordering could also negatively affect the interactions between the redundancy and scheduling mechanisms such as traffic regulators (as with per-flow regulators and interleaved regulators, implemented by TSN asynchronous traffic shaping). Using the network calculus framework, we provide a method of worst-case timing analysis for time-sensitive networks that implement redundancy mechanisms in the general use case, i.e., at end-devices and/or intermediate nodes. We first provide a network calculus toolbox for bounding the burstiness increase and the amount of reordering caused by the elimination function of duplicate packets. We then analyze the interactions with traffic regulators and show that their shaping-for-free property does not hold when placed after a packet elimination function. We provide a bound for the delay penalty when using per-flow regulators and prove that the penalty is not bounded with interleaved regulators. Finally, we use an industrial use-case to show the applicability and the benefits of our findings.

==> 2-prob-statement/2-3-key-solutions.tex <==
\subsection{Key Solutions in this Paper}
%- a way to compute the burstiness increase and the out of order -> toolbox section ...
%- deep analysis of PREF and regulators interactions and the solution of using POF section \begin{itemize}
%- analyze the applicability of the toolbox and POF solution for an industrial use case

In this paper, we provide a set of results for modeling the effects of \ac{PREF} and their interactions with \acp{POF} and \aclp{REG}.
Our results help the network designer in understanding the consequences of using redundancy mechanisms on the latency bounds.
Through a deep analysis of their interactions, we also list the benefits and drawbacks of using regulators and/or \acp{POF} for mitigating the effects of \ac{PREF}.

Our toolbox (Section~\ref{sec:toolbox}) uses the network-calculus framework for modeling the \ac{PREF} in a better way than with the \emph{intuitive} approach.
Specifically, we provide a tight upper-bound of the flow's burstiness at the output of the \ac{PEF} (Theorem~\ref{thm:toolbox:pef-oac}) and on the amount of packet mis-ordering introduced by the redundancy (Theorem~\ref{thm:toolbox:reordering}).
The bound obtained with Theorem~\ref{thm:toolbox:reordering} can be compared to the application's requirements to decide if a \acf{POF} is required to correct the mis-ordering introduced by \ac{PREF}.
Similarly, the network designer can use the burstiness bound from Theorem~\ref{thm:toolbox:pef-oac} to determine if the network elements placed after the \ac{PEF} can support the worst-case traffic.
If so, the result can be combined with other network-calculus results for obtaining an end-to-end latency bound for the flow.
Otherwise, traffic regulators can be used to mitigate the increase of the burstiness.

When regulators coexist with \ac{PREF}, our deep analysis of their interactions (Section~\ref{sec:regulators}) shows that their effects on the latency bounds depend on the type of regulators: \acfp{PFR} can be used after the \ac{PEF} with or without \ac{POF} and a delay penalty is incurred in the latter case; whereas \acfp{IR} like \ac{TSN} \ac{ATS} lead to unbounded delay if placed after a \ac{PEF} without a \ac{POF}.

Finally, the industrial use-case (Section~\ref{sec:volvo}) highlights how our results support the decision making when designing a time-sensitive network with redundancy mechanisms.
%Finally, we highlight the applicability of our result on an industrial use-case, highlighting how the decision making is 

% These results help the network designer when assessing what are the consequences of using \ac{PREF} on the flow
% Theorem~\ref{thm:toolbox:pef-oac} 
% The network designer can 



% Our results help the network designer in understanding what are the expected consequences of \acf{PREF}  

% First we provide 
% They help the network designer in understanding what are the consequences of using redundancy mechanisms on the flow's latency and in-order-delivery requirements. 
% The network elements placed after the \ac{PEF} can support the worst-case traffic and its peak rate.
% Then our results can be used to compute latency and backlog bounds in the third section of Fig.~\ref{fig:prob-statement:three-sections}; and the \ac{ETE} deterministic performances of the network can be obtained.

% Otherwise, undestnad what can be the benefits and drwabacks of using regs and pfo, what benefits to expect etc etc etc
